Ferromagnetic Phase Transitions in Neutron Stars

The ferromagnetic phase in pure neutron matter as well as charge neutral, beta-equilibrated nuclear matter is considered. We employ Quantum Hadrodynamics, a relativistic field theory description of nuclear matter with meson degrees of freedom, and include couplings between the baryon (proton and neutron) magnetic dipole moment as well as between their charge and the magnetic field in the Lagrangian density describing such a system. We vary the strength of the baryon magnetic dipole moment till a non-zero value of the magnetic field, for which the total energy density of the magnetised system is at a minimum, is found. The system is then assumed to be in the ferromagnetic state. The ferromagnetic equation of state is employed to study matter in the neutron star interior. We find that as the density increases the ferromagnetic field does not increase continuously, but exhibit sudden rapid increases. These sudden increases in the magnetic field correspond to shifts between different configurations of the charged particle's Landau levels and can have significant observational consequences for neutron stars. We also found that although the ferromagnetic phase softens the neutron star equation of state it does not significantly alter the star's mass-radius relationship. The properties of magnetised symmetric nuclear matter were also studied. We confirm that magnetised matter tends to be more proton-rich but become more weakly bound for stronger magnetic fields. We show that the behaviour of the compressibility of nuclear matter is influenced by the Landau quantisation and tends to have an oscillatory character as it increases with the magnetic field. The symmetry energy also exhibits similar behaviour.

==> chapBeta.tex <==
\chapter{Ferromagnetism in nuclear  matter}
The aim of this chapter is add charge particles to the description of ferromagnetism in neutron matter to obtain a description of ferromagnetism in beta- and charged equilibrated nuclear and neutron star mater. 
%
%
%
\section{Magnetic interaction with charged particles}
The electromagnetic potential $A^\mu$ couples to both the charge and spin of charged particles. To include both these effects to our description 
\begin{eqnarray}
	\psi{\scriptstyle (x)}\left(-q_p\gamma^\mu A_\mu-\frac{g_p}{2}\bar{\psi}\sigma^{\mu\nu}F_{\mu\nu}\right)\psi{\scriptstyle (x)}\label{chargedcoup}
\end{eqnarray}
is added to the Lagrangian describing protons. For the leptons only 
\begin{eqnarray}
	-\psi_l{\scriptstyle (x)}q_l\gamma^\mu A_\mu\psi_l{\scriptstyle (x)}
\end{eqnarray}
is added since including the second term in (\ref{chargedcoup}) described the \textsl{anomalous} contribution to the magnetic dipole moment of leptons. The anomalous dipole moment has its orgin in higher order interaction of photons with leptons \cite{P+S}. These are however corrections of the order $\hbar$ and thus small compared the possible change in the fermion magnetic dipole moments which are due to the internal structure of the fermions. Thus we will not include the \textsl{anomalous} term to the magnetic field's interaction with the leptons.




%
%
%
\section{Spectrum}
\begin{eqnarray}
	\sqrt{k_z^2+\left(\sqrt{m_p^2+2\,\alpha\,q_p B\left(n+\frac{1}{2}-\alpha\,\frac{\lambda }{2}\right)}+\lambda  g_p B\right)^2}		
\end{eqnarray}
with
\begin{itemize}
\item $k_z(x)$ the momentum in the $z$-direction ,
\item $q_p$ and $g_p$ the proton charge and coupling strength to the magnetic field respectively,
\item $\alpha =\frac{q_p B}{|q_p B|}$ and $\lambda = \pm 1$ representing the two possible orientations of the particle with regards to $B$,
\item $m_n$ denotes the neutron mass, and,
\item $g_{s}$ and $g_v$  the coupling constants for the scalar and vector mesons fields.
\end{itemize}
